Self-Supervised Vision Transformers for Writer Retrieval

While methods based on Vision Transformers (ViT) have achieved state-of-the-art performance in many domains, they have not yet been applied successfully in the domain of writer retrieval. The field is dominated by methods using handcrafted features or features extracted from Convolutional Neural Networks. In this work, we bridge this gap and present a novel method that extracts features from a ViT and aggregates them using VLAD encoding. The model is trained in a self-supervised fashion without any need for labels. We show that extracting local foreground features is superior to using the ViT's class token in the context of writer retrieval. We evaluate our method on two historical document collections. We set a new state-at-of-art performance on the Historical-WI dataset (83.1\% mAP), and the HisIR19 dataset (95.0\% mAP). Additionally, we demonstrate that our ViT feature extractor can be directly applied to modern datasets such as the CVL database (98.6\% mAP) without any fine-tuning.

==> trash.tex <==

% \begin{table}
% \caption{Comparison of Reranking Methods}\label{tab1}
% \begin{center}
% \begin{tabular}{l c@{\hspace{1em}}c@{\hspace{1em}}c@{\hspace{0.25em}}c@{\hspace{1em}}c@{\hspace{0.25em}}c@{\hspace{1em}}c@{\hspace{0.25em}}c@{\hspace{1em}}c@{\hspace{0.25em}}c}
% \toprule
% & \multicolumn{2}{c}{} & \multicolumn{2}{c}{None} & \multicolumn{2}{c}{kRNN} & \multicolumn{2}{c}{Graph} & \multicolumn{2}{c}{SGR}  \\
% Encoding & Features & Stride & mAP & Top1 & mAP & Top1 & mAP & Top1 & mAP & Top1 \\
% \midrule
% Sum & CLS & 224 & 78.5 & 90.0 & 80.5 & 89.0 & 80.9 & 89.0 & 80.2 & 89.0 \\
% Sum & ALL  & 224 & 74.1 & 88.4  & 77.5  & 87.2  & 77.8 & 87.4  & 77.0  & 86.7  \\
% Sum & FG  & 224 & 77.1 & 90.0  & 78.7  & 88.3  & 78.7  & 87.3  & 78.2  & 87.4    \\
% %\midrule
% VLAD & CLS & 224 & 69.3 & 84.0 \\
% VLAD & ALL & 224 & 80.1 & 90.5 & 80.8 & 89.2  & 81.1  & 89.0  & 80.3 & 88.1  \\ 
% VLAD & FG & 224 & 81.4 & 91.1 & 82.0 & 90.1 & 81.9 & 89.1 & 81.7 & 89.4 \\
% \midrule
% Sum & CLS & 56 & 79.4 & 90.6 & 81.2 & 90.3 & 81.2 & \textbf{89.4} & 81.0 & 89.5 \\
% VLAD & FG & 56  & \textbf{82.6} & \textbf{91.9} & \textbf{83.1} & \textbf{90.9} & \textbf{82.5} & 89.1 & \textbf{82.8} & \textbf{90.2} \\
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table}
% \todo{include hisir19 and shorten a bit} In previous works on writer retrieval, a significant improvement in terms of mAP was achieved by reranking. Rather than directly computing the distance between page descriptors, an updated page descriptor is computed by exploiting the similarities between documents in the retrieval list. In this section, we evaluate the impact of several reranking methods on the performance of our baseline implementation. For this, we evaluate k-Reciprocal Nearest Neighbor (kRNN) reranking~\cite{XX}, Graph reranking~\cite{XX}, and Stochastic Graph Reranking (SGR)~\cite{XX} in combination with sum~pooling on the class tokens (CLS), all patch tokens (ALL) and our foreground patch tokens, as well as VLAD with all patch tokens and our foreground patch tokens. 
% For the Graph-reranking we set k1=4, k2=2, L=3 following [Y]. For SGR, [Y] use a value of $\gamma = 0.4$, which we found to heavily reduce our results. We use a much lower value of $\gamma=0.1$. 

% \cref{tab:rerank} shows that all reranking methods improve the mAP, however the Top1 score is reduced. For sum~pooling, the Graph-based reranking produces the best results. Again, for sum~pooling the best results are obtained with the class token (80.9\% mAP), however the improvement (+2.4\% mAP) is less significant than for the patch tokens (+3.7\%) or the foreground tokens (+2.8\%). Despite this, the ranking of features stays the same, indicating this is mainly due to the already higher baseline performance of CLS and FG tokens.

% For VLAD encoding, we found in the previous experiment that using the class token produces poor results. As such, we skip it in this evaluation and only compare patch tokens and foreground tokens. Here, the best results are obtained with the kRNN reranking. Due to higher baseline performance, the impact of reranking is much less significant in this case. For the foreground tokens an improvement of +0.6\% mAP is achieved (82.0\% mAP) whereas for the patch tokens an improvement of 0.7\% mAP to now 80.8\% can be seen. Again, the foreground features consistently outperform all patch tokens regardless of the reranking method. \textbf{!Graph better for VLAD-ALL}

% When reducing the stride to 56, an increase in performance can be observed. sum~pooling with the class tokens achieves 81.2\% mAP, both with kRNN and Graph-based reranking. For VLAD on the foreground tokens, the best results are again achieved with kRNN reranking (83.1\% mAP). Interestingly, the Graph-based reranking actually leads to a reduction in mAP with this configuration and is outperformed by SGR, which in all other cases falls short of the other reranking methods. 


% OLD VERSION OF TAB2
%\begin{table}
%\caption{Comparison of Different Pooling Methods}\label{tab1}
%\begin{center}
%
%\begin{tabular}{cc cc cc cc cc}
%\toprule
%\multicolumn{2}{c}{}& \multicolumn{2}{c}{None} & \multicolumn{2}{c}{kRNN} & \multicolumn{2}{c}{Graph} & \multicolumn{2}{c}{SGR}  \\
%Features & Stride & mAP & Top1 & mAP & Top1 & mAP & Top1 & mAP & Top1 \\
%\midrule
%
%Sum (CLS) & 224 & 78.5 & 90.0 & 80.5 & 89.0 & 80.9 & 89.0 & 80.2 & 89.0 \\
%Sum (CLS) & 56 & 79.4 & 90.6 & 81.2 & 90.3 & 81.2 & \textbf{89.4} & 81.0 & 89.5 \\
%\midrule
%VLAD (FG) & 224 & 81.4 & 91.1 & 82.0 & 90.1 & 81.9 & 89.1 & 81.7 & 89.4 \\
%VLAD (FG) & 56 & \textbf{82.6} & \textbf{91.9} & \textbf{83.1} & \textbf{90.9} & \textbf{82.5} & 89.1 & \textbf{82.8} & \textbf{90.2} \\
%\bottomrule
%\end{tabular}
%
%\end{center}
%\end{table}

% OLD LAYOUT
%\begin{table}
%\caption{Comparison of Different Pooling Methods}\label{tab1}
%\begin{center}%

%\begin{tabular}{l|cc|cc|cc|cc}
%& \multicolumn{2}{c|}{Sum (CLS/224)} & \multicolumn{2}{c|}{Sum (CLS/56)} & \multicolumn{2}{c|}{VLAD (FG/224)} & \multicolumn{2}{c}{VLAD (FG/56)} \\%

%Method & mAP & Top1 & mAP & Top1 & mAP & Top1 & mAP & Top1 \\
%\hline%

%None & 78.5 & \textbf{90.0} & 79.4 & \textbf{90.6} & 81.4 & \textbf{91.1} & 82.6 & \textbf{91.9} \\
%kRNN & 80.5 & 89.0 & \textbf{81.2} & 90.3 & \textbf{82.0} & 90.1 & \textbf{83.1} & 90.9 \\
%Graph & \textbf{80.9} & 89.0 & 81.2 & 89.4 & 81.9 & 89.1 & 82.5 & 89.1 \\
%SGR & 80.2 & 89.0 & 81.0 & 89.5 & 81.7 & 89.4 & 82.8 & 90.2 \\%

%\end{tabular}%

%\end{center}
%\end{table}%




% \subsection{Training Method}

% Our baseline implementation uses AttMask (High) to train our Vision Transformer model. In this section, we investigate other training paradigms methods. For the training dataset, the identity of the writers is known. These writer ids can be used to train the model in a supervised fashion. An alternative approach for supervised training could be treating each document image as their own class, i.e., given a window extracted from a document, the model has to predict the id of the document. We evaluate both of these scenarios, to investigate whether a self-supervised approach is necessary. Additionally, we evaluate two other self-supervised learning methods: iBOT~\cite{} and DINO~\cite{}. 
% We repeat the experiments conducted in the previous two sections for each of these training methods, that is, we evaluate their performance when coupled with sum~pooling and VLAD, and with subsequent reranking applied. 

% namely iBOT and DINO, as well as basic supervised training using either the page id or the writer id as supervision signal. 


% AttMask (High) outperforms the other methods slightly, however, it is worth highlighting that the results are within 1\% mAP of each other. This showcases that our proposed method does not rely on a specific training method.

% [...] 

% supervised training: same parameters as ssl
% maybe no lr scheduler






% \subsection{Training Window Extraction}
% IN this section we evaluate the impact of sampling strategy during training. We compare a SIFT based approach, using 50\% overlap and 87.5\% overlap and no overlap. 

% Todo: Train 0\% overlap, evaluate 
% CLS - SumPooling
% FG - SumPooling
% FG - VLAD
% FG + bVLAD + SGR

% \subsection{Influence of Data Augmentation}
% In this section we evaluate the impact of using morphological operations for data augmentation compared with just using the out-of-the-box augmentations used in other domains. 

% Todo: Evaluieren:
% CLS - SumPooling
% FG - SumPooling
% FG - VLAD
% FG + bVLAD + SGR
